Give Me Your Attention: Dot-Product Attention Considered Harmful for Adversarial Patch Robustness

Neural architectures based on attention such as vision transformers are revolutionizing image recognition. Their main benefit is that attention allows reasoning about all parts of a scene jointly. In this paper, we show how the global reasoning of (scaled) dot-product attention can be the source of a major vulnerability when confronted with adversarial patch attacks. We provide a theoretical understanding of this vulnerability and relate it to an adversary's ability to misdirect the attention of all queries to a single key token under the control of the adversarial patch. We propose novel adversarial objectives for crafting adversarial patches which target this vulnerability explicitly. We show the effectiveness of the proposed patch attacks on popular image classification (ViTs and DeiTs) and object detection models (DETR). We find that adversarial patches occupying 0.5% of the input can lead to robust accuracies as low as 0% for ViT on ImageNet, and reduce the mAP of DETR on MS COCO to less than 3%.

==> tables/untargeted_combo.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Reduction: Kq loss%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \begin{table*}[tb]
        \centering
        \caption{Reduction: Kq loss}
        \footnotesize
        \label{tab: Kq_loss}
        

    \begin{tabular}{cccccccc}\toprule
            && ViT-T & ViT-B & ViT-B-384 & DeiT-T & DeiT-B & DeiT-B-384
            \\\midrule
            $\logsumexp$ & $\logsumexp$ & 0.00 & 0.10 & 2.50 & 0.00 & 19.30 & 39.80\\
        \rowcolor{Gray}$\logsumexp$ & mean & 0.00 \smlt{green}{(-0.00)} & 0.00 \smlt{green}{(--0.10)} & 2.90 \smlt{red}{(+0.40)} & 0.00 \smlt{green}{(-0.00)} & 18.30 \smlt{green}{(--1.00)} & 40.40 \smlt{red}{(+0.60)}\\
        $\logsumexp$ & $\max$ & 0.10 \smlt{red}{(+0.10)} & 15.60 \smlt{red}{(+15.50)} & 26.70 \smlt{red}{(+24.20)} & 1.20 \smlt{red}{(+1.20)} & 27.10 \smlt{red}{(+7.80)} & 45.70 \smlt{red}{(+5.90)}\\
        \rowcolor{Gray}mean & $\logsumexp$ & 0.00 \smlt{green}{(-0.00)} & 0.20 \smlt{red}{(+0.10)} & 2.70 \smlt{red}{(+0.20)} & 0.10 \smlt{red}{(+0.10)} & 17.80 \smlt{green}{(--1.50)} & 40.60 \smlt{red}{(+0.80)}\\
        mean & mean & 0.00 \smlt{green}{(-0.00)} & 0.10 \smlt{green}{(-0.00)} & 3.50 \smlt{red}{(+1.00)} & 0.00 \smlt{green}{(-0.00)} & 17.50 \smlt{green}{(--1.80)} & 39.60 \smlt{green}{(--0.20)}\\
        \rowcolor{Gray}mean & $\max$ & 0.20 \smlt{red}{(+0.20)} & 13.80 \smlt{red}{(+13.70)} & 24.60 \smlt{red}{(+22.10)} & 1.50 \smlt{red}{(+1.50)} & 26.10 \smlt{red}{(+6.80)} & 46.10 \smlt{red}{(+6.30)}\\
        $\max$ & $\logsumexp$ & 0.00 \smlt{green}{(-0.00)} & 3.30 \smlt{red}{(+3.20)} & 5.80 \smlt{red}{(+3.30)} & 0.00 \smlt{green}{(-0.00)} & 36.60 \smlt{red}{(+17.30)} & 45.90 \smlt{red}{(+6.10)}\\
        \rowcolor{Gray}$\max$ & mean & 0.00 \smlt{green}{(-0.00)} & 2.40 \smlt{red}{(+2.30)} & 9.20 \smlt{red}{(+6.70)} & 0.00 \smlt{green}{(-0.00)} & 23.80 \smlt{red}{(+4.50)} & 43.60 \smlt{red}{(+3.80)}\\
        $\max$ & $\max$ & 3.70 \smlt{red}{(+3.70)} & 45.50 \smlt{red}{(+45.40)} & 59.70 \smlt{red}{(+57.20)} & 1.50 \smlt{red}{(+1.50)} & 58.50 \smlt{red}{(+39.20)} & 58.80 \smlt{red}{(+19.00)}\\
        \bottomrule
        \end{tabular}

    \end{table*}
    
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Reduction: Class token%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \begin{table*}[t]
        \centering
        \caption{Reduction: Class token}
        \footnotesize
        \label{tab: Class_token}
        

    \begin{tabular}{cccccccc}\toprule
            && ViT-T & ViT-B & ViT-B-384 & DeiT-T & DeiT-B & DeiT-B-384
            \\\midrule
            $\logsumexp$ & $\logsumexp$ & 0.00 & 0.10 & 1.90 & 0.00 & 13.10 & 40.60\\
        \rowcolor{Gray}$\logsumexp$ & mean & 0.00 \smlt{green}{(-0.00)} & 0.40 \smlt{red}{(+0.30)} & 1.90 \smlt{green}{(-0.00)} & 0.00 \smlt{green}{(-0.00)} & 13.50 \smlt{red}{(+0.40)} & 40.20 \smlt{green}{(--0.40)}\\
        $\logsumexp$ & $\max$ & 0.00 \smlt{green}{(-0.00)} & 24.80 \smlt{red}{(+24.70)} & 43.40 \smlt{red}{(+41.50)} & 0.30 \smlt{red}{(+0.30)} & 21.30 \smlt{red}{(+8.20)} & 47.00 \smlt{red}{(+6.40)}\\
        \rowcolor{Gray}mean & $\logsumexp$ & 0.00 \smlt{green}{(-0.00)} & 0.00 \smlt{green}{(--0.10)} & 2.10 \smlt{red}{(+0.20)} & 0.00 \smlt{green}{(-0.00)} & 12.30 \smlt{green}{(--0.80)} & 38.50 \smlt{green}{(--2.10)}\\
        mean & mean & 0.00 \smlt{green}{(-0.00)} & 0.30 \smlt{red}{(+0.20)} & 2.50 \smlt{red}{(+0.60)} & 0.10 \smlt{red}{(+0.10)} & 11.80 \smlt{green}{(--1.30)} & 40.10 \smlt{green}{(--0.50)}\\
        \rowcolor{Gray}mean & $\max$ & 0.10 \smlt{red}{(+0.10)} & 16.40 \smlt{red}{(+16.30)} & 32.80 \smlt{red}{(+30.90)} & 0.80 \smlt{red}{(+0.80)} & 19.90 \smlt{red}{(+6.80)} & 47.00 \smlt{red}{(+6.40)}\\
        $\max$ & $\logsumexp$ & 0.00 \smlt{green}{(-0.00)} & 0.20 \smlt{red}{(+0.10)} & 1.00 \smlt{green}{(--0.90)} & 0.20 \smlt{red}{(+0.20)} & 23.90 \smlt{red}{(+10.80)} & 50.70 \smlt{red}{(+10.10)}\\
        \rowcolor{Gray}$\max$ & mean & 0.00 \smlt{green}{(-0.00)} & 0.80 \smlt{red}{(+0.70)} & 5.90 \smlt{red}{(+4.00)} & 0.10 \smlt{red}{(+0.10)} & 14.50 \smlt{red}{(+1.40)} & 47.00 \smlt{red}{(+6.40)}\\
        $\max$ & $\max$ & 0.00 \smlt{green}{(-0.00)} & 31.70 \smlt{red}{(+31.60)} & 45.50 \smlt{red}{(+43.60)} & 1.20 \smlt{red}{(+1.20)} & 56.80 \smlt{red}{(+43.70)} & 60.90 \smlt{red}{(+20.30)}\\
        \bottomrule
        \end{tabular}

    \end{table*}


==> tables/untargeted_kq_weight_ablation.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Untargeted - head reduction: logsumexp, layer reduction: logsumexp%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \begin{table*}[tb]
        \centering
        \caption{Untargeted - head reduction: logsumexp, layer reduction: logsumexp
        Waiting for the complete results of tiny models}
        \footnotesize
        \label{tab: untargeted}
        
    \begin{tabular}{lcccccccc}\toprule
            & ViT-T & ViT-S & ViT-B & ViT-B-384 & DeiT-T & DeiT-S & DeiT-B & DeiT-B-384
            \\\midrule
            $\mathcal{L}_{ce}$ pgd 250 $\alpha$=8/255 & 0.10 & 3.60 & 13.50 & 31.20 & 19.80 & 26.10 & 36.00 & 58.80\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq} \quad0.25$ & 0.44 \smlt{red}{(+0.34)} & 2.40 \smlt{green}{(--1.20)} & 5.20 \smlt{green}{(--8.30)} & 20.10 \smlt{green}{(--11.10)} & 17.01 \smlt{green}{(--2.79)} & 28.40 \smlt{red}{(+2.30)} & 36.50 \smlt{red}{(+0.50)} & 56.40 \smlt{green}{(--2.40)}\\
        $\quad + \mathcal{L}_{kq} \quad0.5$ & 0.43 \smlt{red}{(+0.33)} & 2.60 \smlt{green}{(--1.00)} & 5.70 \smlt{green}{(--7.80)} & 18.70 \smlt{green}{(--12.50)} & 15.86 \smlt{green}{(--3.94)} & 29.70 \smlt{red}{(+3.60)} & 36.00 \smlt{green}{(-0.00)} & 56.00 \smlt{green}{(--2.80)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq} \quad0.75$ & 0.20 \smlt{red}{(+0.10)} & 3.90 \smlt{red}{(+0.30)} & 5.60 \smlt{green}{(--7.90)} & 18.20 \smlt{green}{(--13.00)} & 13.10 \smlt{green}{(--6.70)} & 28.50 \smlt{red}{(+2.40)} & 35.80 \smlt{green}{(--0.20)} & 56.20 \smlt{green}{(--2.60)}\\
        $\quad + \mathcal{L}_{kq} \quad1.0$ & 0.50 \smlt{red}{(+0.40)} & 4.60 \smlt{red}{(+1.00)} & 5.00 \smlt{green}{(--8.50)} & 18.00 \smlt{green}{(--13.20)} & 13.10 \smlt{green}{(--6.70)} & 30.80 \smlt{red}{(+4.70)} & 35.50 \smlt{green}{(--0.50)} & 55.10 \smlt{green}{(--3.70)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq*} \quad0.25$ & 0.11 \smlt{red}{(+0.01)} & 2.70 \smlt{green}{(--0.90)} & 5.40 \smlt{green}{(--8.10)} & 17.10 \smlt{green}{(--14.10)} & 16.59 \smlt{green}{(--3.21)} & 24.90 \smlt{green}{(--1.20)} & 37.40 \smlt{red}{(+1.40)} & 57.90 \smlt{green}{(--0.90)}\\
        $\quad + \mathcal{L}_{kq*} \quad0.5$ & 0.32 \smlt{red}{(+0.22)} & 3.20 \smlt{green}{(--0.40)} & 3.60 \smlt{green}{(--9.90)} & 15.20 \smlt{green}{(--16.00)} & 15.97 \smlt{green}{(--3.83)} & 23.30 \smlt{green}{(--2.80)} & 33.80 \smlt{green}{(--2.20)} & 58.40 \smlt{green}{(--0.40)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq*} \quad0.75$ & 0.10 \smlt{green}{(-0.00)} & 3.80 \smlt{red}{(+0.20)} & 3.30 \smlt{green}{(--10.20)} & 14.10 \smlt{green}{(--17.10)} & 14.00 \smlt{green}{(--5.80)} & 21.60 \smlt{green}{(--4.50)} & 33.20 \smlt{green}{(--2.80)} & 57.40 \smlt{green}{(--1.40)}\\
        $\quad + \mathcal{L}_{kq*} \quad1.0$ & 0.30 \smlt{red}{(+0.20)} & 4.80 \smlt{red}{(+1.20)} & 2.60 \smlt{green}{(--10.90)} & 13.00 \smlt{green}{(--18.20)} & 11.70 \smlt{green}{(--8.10)} & 22.10 \smlt{green}{(--4.00)} & 33.70 \smlt{green}{(--2.30)} & 57.20 \smlt{green}{(--1.60)}\\
        \rowcolor{Gray}$+$ Momentum & 0.00 & 0.10 & 3.10 & 13.20 & 1.50 & 3.20 & 16.80 & 41.70\\
        $\quad + \mathcal{L}_{kq} \quad0.25$ & 0.00 \smlt{green}{(-0.00)} & 0.10 \smlt{green}{(-0.00)} & 0.50 \smlt{green}{(--2.60)} & 3.80 \smlt{green}{(--9.40)} & 0.64 \smlt{green}{(--0.86)} & 4.80 \smlt{red}{(+1.60)} & 16.70 \smlt{green}{(--0.10)} & 38.90 \smlt{green}{(--2.80)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq} \quad0.5$ & 0.00 \smlt{green}{(-0.00)} & 0.30 \smlt{red}{(+0.20)} & 0.40 \smlt{green}{(--2.70)} & 3.40 \smlt{green}{(--9.80)} & 0.00 \smlt{green}{(--1.50)} & 4.10 \smlt{red}{(+0.90)} & 18.70 \smlt{red}{(+1.90)} & 36.90 \smlt{green}{(--4.80)}\\
        $\quad + \mathcal{L}_{kq} \quad0.75$ & 0.00 \smlt{green}{(-0.00)} & 0.90 \smlt{red}{(+0.80)} & 0.20 \smlt{green}{(--2.90)} & 3.00 \smlt{green}{(--10.20)} & 0.10 \smlt{green}{(--1.40)} & 4.00 \smlt{red}{(+0.80)} & 17.80 \smlt{red}{(+1.00)} & 38.90 \smlt{green}{(--2.80)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq} \quad1.0$ & 0.00 \smlt{green}{(-0.00)} & 1.00 \smlt{red}{(+0.90)} & 0.10 \smlt{green}{(--3.00)} & 2.50 \smlt{green}{(--10.70)} & 0.00 \smlt{green}{(--1.50)} & 3.80 \smlt{red}{(+0.60)} & 19.30 \smlt{red}{(+2.50)} & 39.80 \smlt{green}{(--1.90)}\\
        $\quad + \mathcal{L}_{kq*} \quad0.25$ & 0.00 \smlt{green}{(-0.00)} & 0.10 \smlt{green}{(-0.00)} & 0.40 \smlt{green}{(--2.70)} & 3.30 \smlt{green}{(--9.90)} & 0.22 \smlt{green}{(--1.28)} & 2.60 \smlt{green}{(--0.60)} & 14.10 \smlt{green}{(--2.70)} & 40.30 \smlt{green}{(--1.40)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq*} \quad0.5$ & 0.00 \smlt{green}{(-0.00)} & 0.70 \smlt{red}{(+0.60)} & 0.30 \smlt{green}{(--2.80)} & 3.60 \smlt{green}{(--9.60)} & 0.00 \smlt{green}{(--1.50)} & 2.10 \smlt{green}{(--1.10)} & 15.70 \smlt{green}{(--1.10)} & 39.90 \smlt{green}{(--1.80)}\\
        $\quad + \mathcal{L}_{kq*} \quad0.75$ & 0.00 \smlt{green}{(-0.00)} & 1.10 \smlt{red}{(+1.00)} & 0.30 \smlt{green}{(--2.80)} & 2.30 \smlt{green}{(--10.90)} & 0.00 \smlt{green}{(--1.50)} & 2.00 \smlt{green}{(--1.20)} & 12.00 \smlt{green}{(--4.80)} & 39.60 \smlt{green}{(--2.10)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq*} \quad1.0$ & 0.00 \smlt{green}{(-0.00)} & 1.30 \smlt{red}{(+1.20)} & 0.10 \smlt{green}{(--3.00)} & 1.90 \smlt{green}{(--11.30)} & 0.00 \smlt{green}{(--1.50)} & 1.80 \smlt{green}{(--1.40)} & 13.10 \smlt{green}{(--3.70)} & 40.60 \smlt{green}{(--1.10)}\\
        \bottomrule
        \end{tabular}

    \end{table*}


==> tables/untargeted_stepsize_4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Untargeted - head reduction: logsumexp, layer reduction: logsumexp%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

        \begin{table*}[t]
        \centering
        \caption{Untargeted - head reduction: logsumexp, layer reduction: logsumexp}
        \footnotesize
        \label{tab: untargeted}
        

    \begin{tabular}{lcccccccc}\toprule
            & ViT-T & ViT-S & ViT-B & ViT-B-384 & DeiT-T & DeiT-S & DeiT-B & DeiT-B-384
            \\\midrule
            $\mathcal{L}_{ce}$ pgd 250 $\alpha$=4/255 & 2.00 & 13.90 & 20.40 & 40.50 & 27.30 & 38.60 & 44.30 & 62.30\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq} \quad0.25$ & 3.70 \smlt{red}{(+1.70)} & 10.60 \smlt{green}{(--3.30)} & 11.60 \smlt{green}{(--8.80)} & 28.40 \smlt{green}{(--12.10)} & 27.10 \smlt{green}{(--0.20)} & 39.40 \smlt{red}{(+0.80)} & 44.80 \smlt{red}{(+0.50)} & 60.30 \smlt{green}{(--2.00)}\\
        $\quad + \mathcal{L}_{kq} \quad0.5$ & 3.00 \smlt{red}{(+1.00)} & 11.90 \smlt{green}{(--2.00)} & 9.90 \smlt{green}{(--10.50)} & 26.60 \smlt{green}{(--13.90)} & 27.20 \smlt{green}{(--0.10)} & 40.20 \smlt{red}{(+1.60)} & 45.80 \smlt{red}{(+1.50)} & 60.00 \smlt{green}{(--2.30)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq} \quad0.75$ & 2.60 \smlt{red}{(+0.60)} & 11.30 \smlt{green}{(--2.60)} & 9.60 \smlt{green}{(--10.80)} & 25.70 \smlt{green}{(--14.80)} & 26.30 \smlt{green}{(--1.00)} & 41.50 \smlt{red}{(+2.90)} & 46.10 \smlt{red}{(+1.80)} & 59.70 \smlt{green}{(--2.60)}\\
        $\quad + \mathcal{L}_{kq} \quad1.0$ & 3.20 \smlt{red}{(+1.20)} & 12.30 \smlt{green}{(--1.60)} & 9.40 \smlt{green}{(--11.00)} & 25.10 \smlt{green}{(--15.40)} & 26.00 \smlt{green}{(--1.30)} & 40.40 \smlt{red}{(+1.80)} & 45.70 \smlt{red}{(+1.40)} & 60.10 \smlt{green}{(--2.20)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq*} \quad0.25$ & 1.80 \smlt{green}{(--0.20)} & 11.90 \smlt{green}{(--2.00)} & 11.30 \smlt{green}{(--9.10)} & 25.40 \smlt{green}{(--15.10)} & 26.20 \smlt{green}{(--1.10)} & 36.20 \smlt{green}{(--2.40)} & 44.70 \smlt{red}{(+0.40)} & 61.20 \smlt{green}{(--1.10)}\\
        $\quad + \mathcal{L}_{kq*} \quad0.5$ & 1.30 \smlt{green}{(--0.70)} & 11.40 \smlt{green}{(--2.50)} & 9.40 \smlt{green}{(--11.00)} & 25.60 \smlt{green}{(--14.90)} & 24.80 \smlt{green}{(--2.50)} & 35.50 \smlt{green}{(--3.10)} & 44.20 \smlt{green}{(--0.10)} & 60.00 \smlt{green}{(--2.30)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq*} \quad0.75$ & 1.90 \smlt{green}{(--0.10)} & 11.90 \smlt{green}{(--2.00)} & 8.20 \smlt{green}{(--12.20)} & 23.50 \smlt{green}{(--17.00)} & 22.70 \smlt{green}{(--4.60)} & 35.20 \smlt{green}{(--3.40)} & 45.00 \smlt{red}{(+0.70)} & 61.70 \smlt{green}{(--0.60)}\\
        $\quad + \mathcal{L}_{kq*} \quad1.0$ & 1.30 \smlt{green}{(--0.70)} & 13.60 \smlt{green}{(--0.30)} & 8.40 \smlt{green}{(--12.00)} & 22.90 \smlt{green}{(--17.60)} & 22.70 \smlt{green}{(--4.60)} & 35.80 \smlt{green}{(--2.80)} & 46.80 \smlt{red}{(+2.50)} & 62.09 \smlt{green}{(--0.21)}\\
        \rowcolor{Gray}$+$ Momentum & 0.00 & 0.60 & 5.30 & 18.40 & 7.40 & 9.80 & 22.50 & 47.40\\
        $\quad + \mathcal{L}_{kq} \quad0.25$ & 0.00 \smlt{green}{(-0.00)} & 0.80 \smlt{red}{(+0.20)} & 1.50 \smlt{green}{(--3.80)} & 7.40 \smlt{green}{(--11.00)} & 4.40 \smlt{green}{(--3.00)} & 9.40 \smlt{green}{(--0.40)} & 22.50 \smlt{green}{(-0.00)} & 43.60 \smlt{green}{(--3.80)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq} \quad0.5$ & 0.00 \smlt{green}{(-0.00)} & 1.70 \smlt{red}{(+1.10)} & 1.10 \smlt{green}{(--4.20)} & 7.50 \smlt{green}{(--10.90)} & 3.90 \smlt{green}{(--3.50)} & 9.80 \smlt{green}{(-0.00)} & 24.70 \smlt{red}{(+2.20)} & 44.10 \smlt{green}{(--3.30)}\\
        $\quad + \mathcal{L}_{kq} \quad0.75$ & 0.00 \smlt{green}{(-0.00)} & 2.20 \smlt{red}{(+1.60)} & 1.30 \smlt{green}{(--4.00)} & 7.90 \smlt{green}{(--10.50)} & 2.50 \smlt{green}{(--4.90)} & 10.70 \smlt{red}{(+0.90)} & 23.60 \smlt{red}{(+1.10)} & 45.60 \smlt{green}{(--1.80)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq} \quad1.0$ & 0.00 \smlt{green}{(-0.00)} & 3.10 \smlt{red}{(+2.50)} & 0.80 \smlt{green}{(--4.50)} & 7.70 \smlt{green}{(--10.70)} & 2.20 \smlt{green}{(--5.20)} & 10.70 \smlt{red}{(+0.90)} & 22.90 \smlt{red}{(+0.40)} & 44.60 \smlt{green}{(--2.80)}\\
        $\quad + \mathcal{L}_{kq*} \quad0.25$ & 0.00 \smlt{green}{(-0.00)} & 0.60 \smlt{green}{(-0.00)} & 1.60 \smlt{green}{(--3.70)} & 5.90 \smlt{green}{(--12.50)} & 4.00 \smlt{green}{(--3.40)} & 7.70 \smlt{green}{(--2.10)} & 20.70 \smlt{green}{(--1.80)} & 45.70 \smlt{green}{(--1.70)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq*} \quad0.5$ & 0.00 \smlt{green}{(-0.00)} & 0.90 \smlt{red}{(+0.30)} & 1.10 \smlt{green}{(--4.20)} & 5.10 \smlt{green}{(--13.30)} & 2.80 \smlt{green}{(--4.60)} & 7.90 \smlt{green}{(--1.90)} & 20.40 \smlt{green}{(--2.10)} & 44.80 \smlt{green}{(--2.60)}\\
        $\quad + \mathcal{L}_{kq*} \quad0.75$ & 0.00 \smlt{green}{(-0.00)} & 1.40 \smlt{red}{(+0.80)} & 0.80 \smlt{green}{(--4.50)} & 3.90 \smlt{green}{(--14.50)} & 1.90 \smlt{green}{(--5.50)} & 6.80 \smlt{green}{(--3.00)} & 21.10 \smlt{green}{(--1.40)} & 47.00 \smlt{green}{(--0.40)}\\
        \rowcolor{Gray}$\quad + \mathcal{L}_{kq*} \quad1.0$ & 0.00 \smlt{green}{(-0.00)} & 2.00 \smlt{red}{(+1.40)} & 0.60 \smlt{green}{(--4.70)} & 3.30 \smlt{green}{(--15.10)} & 2.00 \smlt{green}{(--5.40)} & 7.30 \smlt{green}{(--2.50)} & 21.30 \smlt{green}{(--1.20)} & 46.37 \smlt{green}{(--1.03)}\\
        \bottomrule
        \end{tabular}

    \end{table*}

